Analyzing Neural Jacobian Methods in Applications of Visual Servoing and Kinematic Control

Designing adaptable control laws that can transfer between different robots is a challenge because of kinematic and dynamic differences, as well as in scenarios where external sensors are used. In this work, we empirically investigate a neural networks ability to approximate the Jacobian matrix for an application in Cartesian control schemes. Specifically, we are interested in approximating the kinematic Jacobian, which arises from kinematic equations mapping a manipulator's joint angles to the end-effector's location. We propose two different approaches to learn the kinematic Jacobian. The first method arises from visual servoing where we learn the kinematic Jacobian as an approximate linear system of equations from the k-nearest neighbors for a desired joint configuration. The second, motivated by forward models in machine learning, learns the kinematic behavior directly and calculates the Jacobian by differentiating the learned neural kinematics model. Simulation experimental results show that both methods achieve better performance than alternative data-driven methods for control, provide closer approximations to the proper kinematics Jacobian matrix, and on average produce better-conditioned Jacobian matrices. Real-world experiments were conducted on a Kinova Gen-3 lightweight robotic manipulator, which includes an uncalibrated visual servoing experiment, a practical application of our methods, as well as a 7-DOF point-to-point task highlighting that our methods are applicable on real robotic manipulators.

==> at_submission/introduction.tex <==
\section{Introduction} \label{sec:introduction}


%Gradient information, or more specifically Jacobian information, has a variety of applications in machine learning and robotics. Many state-of-the-art optimizers utilize previously calculated gradients for adapting learning rates and search directions to train complex learning systems \cite{ruder2016overviewsgdoptimizers}.
This work focuses on learning the kinematics Jacobian, which arises from a manipulator's forward kinematic equations. Forward kinematics describes the location of a manipulator's end-effector $x = f(q)$ where $f$ is the manipulator's kinematic equations, $x\in \mathbf{R}^m$ is the end-effector, and $q\in\mathbf{R}^n$ are the joint angles. Differentiating with respect to time describes the velocity relation between joints and end-effector $J(q)\dot{q} = \dot{x}$ where $J(q) \in R^{m \times n}$ is the kinematic Jacobian. In robotic applications, the kinematic Jacobian can be useful for controlling robots, such as in Cartesian control schemes \cite{craig1989IntroRobotics}. These classical controllers are often preferred in practice because of their well-understood behavior. This contrasts with alternative control approaches, such as those from machine learning, which can be more black-box or volatile in practice for control \cite{henderson2018DeepRL}.

However, calculating the true Jacobian can be difficult in practice for less controlled environments. One reason is due to uncertainty in the kinematics or dynamics of the robotic system. This can arise in object manipulations with robotic fingers where all fingers impose complex-to-model parallel-kinematics \cite{jagersand1996acquiringvismodel}. Another reason is that the introduction of external sensory information changes the structure of the Jacobian. An example of this is visual servoing (VS), where an analytic Jacobian exists but can be difficult to calculate in practice \cite{hitchinson1996tutorialVS}. In these situations, an adaptive learning approach can be beneficial and can help enable the application of robots in less controlled settings \cite{hitchinson1996tutorialVS,jun2019visualgeometric}. 


%A number of Jacobian approximation approaches have been proposed in literature such as in the area of uncalibrated visual servoing (UVS). The earliest works focused on finite differences with online updates to the Jacobian \citep{jagersand96visualservoing,piepmeir2004UDVS,qian2002kalmanuvs}. Researchers sought to improve these approximation by proposing global techniques utilizing collected information from the robot's state information\cite{farahmand2007globaluvs} or hybrid methods combining several  \cite{music2014ComparingUVS}. %These previous global methods \vzhang{have not otherwise considered function approximators to achieve similar goals instead choosing non-parametric models (this part seems unclear to me)}.
For an alternative solution, we argue in favor of data-driven learning methods that learn to predict the kinematic Jacobian. The advantage of this perspective, as opposed to alternatives like end-to-end learning \cite{levine2016endtoend}, is that one can analyze the predicted Jacobian despite the black-box nature of the prediction mechanism. Specifically, we propose two methods based on neural networks trained to predict the Jacobian matrix, specifically with an application for kinematic control schemes in mind. Our first method predicts the Jacobian matrix directly by utilizing a loss function based on the robot's equations of motion. It is motivated by previous work in uncalibrated visual servoing \cite{farahmand2007globaluvs}. We refer to this as the \textit{Neural Jacobian} method.
The second method predicts the forward kinematics, and the Jacobian is recovered with back-propagation. We refer to this forward model approach as the \textit{Neural Kinematics} method. 

The second method predicts the forward kinematics and the Jacobian is recovered with back-propagation. We refer to this forward model approach as the \textit{Neural Kinematics} method.  % %The robot arm equations of motion our defined by differentiating $f(q)$ with respect to time:
%\begin{equation*}
%    \dot{x} = J(q) \dot{q}.
%\end{equation*}
%Here, $\dot{x} \in \mathbf{R}^{m}$ refers to the Cartesian velocity of the tool-tip, or end-effector for the rest of the paper, and  $\dot{q} \in \mathbf{R}^{n}$ refers to the joint angle velocities. The robot's Jacobian $J(q)$  is the partial derivatives of forward kinematics with respect to the robot joint coordinates. $J(q)$ represents the relation between $\dot{q}$ and $\dot{x}$.



%; variations of this approach have been previously studied \cite{farahmand2007globaluvs,zhao2009NNmultifingerJacobian,lyu2018NNvisionjacobianpred,lyu2020datadrivenLearningofJacobian}. We refer to this method as the \textit{Neural Jacobian} in this paper. The second method predicts the forward kinematics and we recover the Jacobian with back-propagation. We refer to this forward model approach as the \textit{Neural Kinematics} method.
In our experiments, we study both methods in a setting of \textit{ab initio learning} where the robot does not have a-priori knowledge of it's own rigid body and must learn to control itself through interacting with the environment \cite{Censi2013BootstrappingV}. We  evaluate our controllers on set-point reaching tasks in extensive simulation experiments. The objective of these tasks is to move our robot's end-effector towards a target $x^{*} \in \mathbf{R}^{m}$. We analyze several aspects of the Jacobian matrices from our control tasks and find that our neural methods are generally closer approximations to alternative learning methods and can be better behaved on average compared to the alternative ab initio approaches considered. We then provide proof-of-concept applications of our methods on a Kinova Gen-3 light robot (Kinova) in a 2-DOF visual servoing task and on the full 7-DOF of the manipulator in it's coordinate system \cite{kinova}. We focus on the general case of kinematic control, excluding analyzing singularity configurations which, to our knowledge, have non-trivial problems warranting special consideration \cite{consistentNullspac1993Chen,overviewNullspace2015dietrich}.
%Our contributions :
%\begin{enumerate}
    
%    \item We propose two approaches for learning a robot's Jacobian matrix both directly and as a by-product of learning the underlying functional relationship for describing a robot's pose.
%    \item We showed that in well-conditioned settings our methods exceed baselines, but in more complex settings performances results varied depending on target distance.  
%    \item We compare our method to two finite difference approaches, and a non-parameteric local linear alternative. In general, we find our neural methods can recover the Jacobian better.
%\end{enumerate}

In Section~\ref{sec:background} we provide pertinent background information. Section~\ref{sec:methodology} discusses our proposed methods in detail. In Section~\ref{sec:experiments} we report our experimental results in simulation and on the Kinova manipulator.  Section~\ref{sec:relatedwork} discusses related work to this research.  We conclude and discuss future research directions in Section~\ref{sec:conclusion}.%



==> at_submission/relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}
In our work, both of our methods are motivated from research in both machine learning and robotics. As such, we discuss work from robotics literature for Jacobian prediction which motivated our Neural Jacobian Method. We then discuss work on function approximation theory and it's applications from machine learning which motivates our Neural Kinematics approach. 

\subsection{Approximate Jacobians in Robotics}


%paragraph 2 uvs related previous work
One area Jacobian approximations are particularly applicable is in the area of \textit{uncalibrated visual servoing}. Researchers have previously studied both local and global approaches. Local methods typically use a finite difference approximation that can be updated online, such as with Broyden's method \citep{jagersand96visualservoing,jagersand1997experimentalevalUVS}, recursive least squares update \citep{piepmeir2004UDVS}, or Kalman filters \citep{music2014ComparingUVS,qian2002kalmanuvs}. These methods are convenient as they are easy to interpret and have local convergence guarantees \cite{nematollahi2009generalizedcontrolawsIBVS}. A limitation though, is they do not remember the information collected while following a trajectory and fail to converge toward distant targets. To mitigate this, global methods attempt to utilize information of the entire workspace to increase performance stability. Previous research has considered non-parametric methods like k-nearest neighbor to combine information of the robotic system for Jacobian estimates \cite{farahmand2007globaluvs}. Our work is most closely related to these global approximations as we attempt to predict Jacobians for the robots entire workspace, but differ by amortizing the online optimization of the Jacobian by training a neural network to make the predictions.

%deep learning specific stuff
%Specifically for deep learning approaches for uncalibrated visual servoing, to our knowledge no previous work has focused on methods to learn the Jacobian matrix. Instead, much research has focused on directly predicting the pose from robot and image information. This has included fully-connected networks which instead predicted the joint-angles to derive control schemes \citep{wells1996visionbasedpositionNN,klobucar2008UVSnn}. For convolutional neural networks this has included a supervised learning approach for eye-in-hand configurations where synthetic training data is generated by transforming images with homography's formed from a desired robot's pose transformation \cite{bateux2018traindeepNNforVS}. In relation to previous work, our Neural Kinematic model is most similar to those which utilized fully-connected networks where we differ by utilizing the forward prediction for recovering the Jacobian matrix.

Although to our knowledge our Neural Jacobian formulation is novel, variations of the Neural Jacobian method have previously been proposed in the literature. The Neural Jacobian method was, originally proposed and experimented on for  multi-finger robotic systems \cite{zhao2009NNmultifingerJacobian}. It was later applied in the context of visual servoing \cite{lyu2018NNvisionjacobianpred}. More recently, it was considered in the same context as ours, but optimized with a two stage gradient-free learning approach \cite{lyu2020datadrivenLearningofJacobian}. These works primarily focused on developing convergence theory and on the method itself. One key difference of these works compared to ours is assuming access to the velocity information whereas we only utilize pose information. In our work, we compare our approach to several alternative approaches on a diverse set of trajectories of varying distances, as well as studying the optimization for the neural network by fitting the inverse relationship. %We did not directly compare to the work of Lyu et. al. \cite{lyu2020datadrivenLearningofJacobian} because, to our knowledge, they did not release source code for reproducibility. 

\subsection{Approximating Gradients with Function Approximators}

%start with how lots of areas of machine learning just take this for granted
In many areas of machine learning, end-to-end gradient propagation implicitly assumes a sub-network will provide meaningful information to the rest of the system being optimized. In research areas such as generative adversarial networks, gradients are calculated with respect to the discriminator network to optimize the generator \cite{goodfellow2014GANS}. This idea appears in reinforcement learning in both model-based and model-free reinforcement learning where gradients are calculated with respect to the neural network approximation of the transition dynamics or value function \cite{lillicrap2016ddpg,gal2016improving}. Most closely tied to our work is the work of Jordan et. al. \cite{jordan1989GenericConstraints} where they explicitly discuss the utilization of an approximate Jacobian. Our work differs as we consider directly using this approximate Jacobian for control whereas they utilize it to optimize a sub-network for control more typical in deep learning. 

Although not often explicitly talked about, early deep learning theory does suggest these assumptions of a neural networks gradients are warranted. For a variety of activation functions, neural network theory has shown that fully connected neural networks can approximate both the function and it's derivatives with as few as one hidden layer \cite{hornik1990universalapproximatorandderivs,hornik95degreeof}. Similar results were found for alternative approaches for function approximation such as radial basis networks \cite{maiduy200rbfderivapprox}. These theoretical results provide a base on which our Neural Kinematics method has a chance of being successful for approximating robotic manipulator motions.  


==> draft_files/methodology_draft.tex <==
\section{Methodology} \label{sec:methodology}

In this section we describe both of the approaches we considered in our work. The first approach is a more natural approach with how function approximators have been used by directly predicting the interaction matrix. The second indirectly learns the interaction matrix by training the function approximator to predict the pose of the robot. 

In this section, we use q for referring to the joint angles fo the robot, x for the features tracked on our manipulator, $x^{*}$ for the target features, $q^{*}$ for the target pose, $\theta$ for the model parameters. We also use $s$ for robot state which can include the $x$, $q$, $\dot{q}$ which is joint velocity, and $x^{*}$.

\subsection{Predicting the Jacobian}

In our direct approach for learning the interaction matrix we use the following objective:
\begin{equation}
    \min_{\theta} || \Delta x - J_{\theta}(s) \Delta q ||_{2}^{2},
\end{equation}
where $\Delta x = x_{t+1} - x_{t}$ and $\Delta q = q_{t+1} - q_{t}$ for subsequent time steps $t$. This approach has previously been considered in several works to optimize an approximate $\hat{J}$ <cite> or to update the the approximation online <cite>. It comes from numerical methods which assumes that under a sufficiently small change in time the finite difference relations can be approximated as $\Delta x \approx J(q_{t}) \Delta q$. 

One may notice that we provide $s$ to our $J_{\theta}(s)$  as opposed to just our joint angles $q$. This choice is because using only $q$ with this approach does not necessarily work with the loss function which indirectly depends on $\Delta q$. To account for this, we found including position $x$ and current joint velocities $\dot{q}$ along with the joint angles $q$ helped the function approximator to provide a better inference of $J_{\theta}(s)$ \textbf{part of my experiments are  to verify the feature choices...i think it should be the case though since the target doesn't play into the above optimization at all}.

One additional consideration is that in the above objective we cannot necessarily say just because $J_{\theta}$ fits well in the finite difference relation that taking the inverse will be a good approximation as well. To see if this relationship does matter we expanded our objective to fit both relationships with our predicted $J_{\theta}$:
\begin{equation}
    \min_{\theta} || \Delta X - J_{\theta} * \Delta q ||_{2}^{2} + || \Delta q -  J_{\theta}^{\dagger} \Delta x ||_{2}^{2}
\end{equation}

Here we introduce the pseudo inverse $J_{\theta}^{\dagger} = (J_{\theta} J_{\theta}^{T})^{-1} J_{\theta}^{T}$ and dropped the input s. For those unfamiliar, it is feasible to differentiate with respect to the pseudo inverse <cite>.

\textbf{Everything above I have run experiments on in simulation in robot space at this point and they seem to work OK. this next paragraph is another way to optimize the above objective, I need to actually see if this works, I suspect it will...but who's to say}

Alternatively, to force dependence only on q, we could follow <cite> and instead minimize the loss on the k-nearest neighbors for given joint angles
\begin{equation}
    \min_{\theta} \sum_{i=1}^{N} \sum_{j=1}^{N} || \Delta x_{ij} - J_{\theta}(q) * \Delta q_{ij} ||_{2}^{2},
\end{equation}
where here we use $ij$ to refer to the finite difference of $\Delta x_{ij} = x_{i} - x_{j}$ and $\Delta q_{ij} = q_{i} - q_{j}$ for each nearest neighbor to the joint angles $q$. Here, we only predict a single $J_{\theta}$ which should fit well to all nearest neighbors. The intuition is the best fitting hyperplane around the surrounding points is a close approximation to the true Jacobian in this way. The difference in this case from their work is they optimize J online at each step, effectively making their method non-parametric by maintaining a memory of all previous interactions as opposed to function approximation method.




\subsection{Predicting the Pose}

Fundamentally in visual servoing, it can be assumed that there does exist some optimal function $f^{*}$ representing the true relationship between the robot and image features. With this observation, our second method attempts to learn this directly. If we let $f_{\theta}(q) = \hat{x}$ represent prediction of the true underlying function, we can optimize this model with supervised learning with any appropriate loss by just collecting $(x, q)$ tuples from the robot-camera system and optimizing the relationship between joint angles $q$ and pose $x$. In our experiments we just use the mean squared error:
\begin{equation}
    \min_{\theta} || x - f_{\theta}(q)||^{2}_{2}
\end{equation}

We define $f^{i}_{\theta}(q)$ as predicting a particular dimension of our multi-dimensional output where each corresponding to an image feature $x^{i}$. Once our approximator $f_{\theta}$ has been optimized, we can then directly calculate the interaction matrix by differentiating with respect to q for each output dimension:
\begin{equation}
       J = \begin{pmatrix}
        \frac{\partial f_{\theta}^{1}}{\partial q_{1}} & \frac{\partial f_{\theta}^{1}}{\partial q_{2}} ... \frac{\partial f_{\theta}^{1}}{\partial q_{n}}\\[\jot]
        \frac{\partial f_{\theta}^{2}}{\partial q_{1}} & \frac{\partial f_{\theta}^{2}}{\partial q_{2}} ... \frac{\partial f_{\theta}^{2}}{\partial q_{n}}\\[\jot]
    \end{pmatrix}
\end{equation}

Intuitively this is an appropriate assumption on the behavior of a good function approximator that the partial derivatives of it should reflect the underlying function as well. This idea has been used in a variety of areas of machine learning such as the deterministic gradient update rule, Generative adversarial networks, style transfer for images, and other machine learning models which learn end-to-end. To our knowledge, this has not been considered in the visual servoing setting, although predicting pose has been considered previously. 


\subsection{Incorporating Temporal difference Jacobians}

\textbf{This section is an extension to the above ideas. It is untested, and to my knowledge not really grounded in anything theoretically sound.  I'm not so confident it will work (setting it up is fairly easy with my codebase so far though....actually i think teeeechnically (if this...worked for some reason) I could really use it for both the above methods. Again, no way to really know if it would help but it's do-able}

Motivated by temporal difference learning, we can alternatively keep an exponentially weighted sum of previously predict Jacobians as an eligibility trace $e_{t}$ of previous predictions:

\begin{equation}
    J^{t} = \sum_{k=1}^{t} \lambda^{t-k} J_{k}
\end{equation}

We can then rewrite the above as the eligibility trace instead
\begin{equation}
    e_{t+1} = J_{t+1} + \lambda e_{t}
\end{equation}

The intuition behind why we might consider such an update is that at each step our Jacobian encodes the best direction in a linearization of the system to move the robot to the target position. This means that each previous prediction may still provide useful information on servoing the robot in the correct direction. Particularly with function approximators it may be the case when our pose estimations are inaccurate in certain regions of the workspace, and trusting previous predictions may be the better decision to continue servoing towards a desired pose.

To further help mitigate the negative influence of inaccurate predictions we can combine the above update using the previously proposed broyden update to modify our eligibility trace online to better guide our average:
\begin{equation}
    e'_{t} = e_{t} + \frac{\alpha}{||\Delta q||^{2}} (\Delta x - e_{t}\Delta q) \otimes\Delta q
\end{equation}
This update has previously been used for updating the predicted Jacobian online for a local uncalibrated visual servoing method. The idea here is after moving the robot with the predicted $\dot{q}$ we can modify our running average in such a way that shapes it's information to still guide us towards the target pose $x^{*}$ 

We then would update our trace as follows:
\begin{equation}
    e_{t+1} = J_{t+1} + \lambda e'_{t}
\end{equation}

The further intuition on why this might work is that as we collect our eligibility trace, previously useful information encoded is no longer helpful. To counter that effect, the Broyden update provides a means to modify the information we have collected in the trajectory to (hopefully) guide our Jacobian estimations in such a way to continue being useful.


==> draft_files/single_and_multipoint_tables.tex <==
\begin{table}[] 
\begin{tabular}{crrrrr}
\multicolumn{1}{l}{}                                     & \multicolumn{5}{c}{\textbf{Initial Euclidean Distance}}                                                                                                                                                       \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}}                     & \multicolumn{1}{c|}{\textit{0.0 - 0.5}} & \multicolumn{1}{c|}{\textit{0.5 - 1.0}} & \multicolumn{1}{c|}{\textit{1.0 - 1.5}} & \multicolumn{1}{c|}{\textit{1.5 - 2.0}} & \multicolumn{1}{c|}{\textit{Overall}} \\ \hline
\multicolumn{1}{|c|}{\textit{Inverse Jacobian}}          & \multicolumn{1}{r|}{100.00}             & \multicolumn{1}{r|}{94.93}              & \multicolumn{1}{r|}{83.30}              & \multicolumn{1}{r|}{76.0}               & \multicolumn{1}{r|}{88.45}            \\ \hline
\multicolumn{1}{|c|}{\textit{Broyden}}                   & \multicolumn{1}{r|}{\textbf{100.00}}    & \multicolumn{1}{r|}{51.93}              & \multicolumn{1}{r|}{18.90}              & \multicolumn{1}{r|}{0.0}                & \multicolumn{1}{r|}{37.00}            \\ \hline
\multicolumn{1}{|c|}{\textit{Finite Difference}}         & \multicolumn{1}{r|}{98.11}              & \multicolumn{1}{r|}{39.61}              & \multicolumn{1}{r|}{17.58}              & \multicolumn{1}{r|}{2.4}                & \multicolumn{1}{r|}{31.91}            \\ \hline
\multicolumn{1}{|c|}{\textit{Local Linear}}              & \multicolumn{1}{r|}{86.79}              & \multicolumn{1}{r|}{66.43}              & \multicolumn{1}{r|}{37.58}              & \multicolumn{1}{r|}{12.8}               & \multicolumn{1}{r|}{50.36}            \\ \hline
\multicolumn{1}{|c|}{\textit{Multitask Neural Jacobian}} & \multicolumn{1}{r|}{99.06}              & \multicolumn{1}{r|}{74.64}              & \multicolumn{1}{r|}{35.82}              & \multicolumn{1}{r|}{3.2}                & \multicolumn{1}{r|}{52.82}            \\ \hline
\multicolumn{1}{|c|}{\textit{Neural Jacobian}}           & \multicolumn{1}{r|}{99.06}              & \multicolumn{1}{r|}{\textbf{84.54}}     & \multicolumn{1}{r|}{\textbf{65.71}}     & \multicolumn{1}{r|}{25.6}               & \multicolumn{1}{r|}{\textbf{71.45}}   \\ \hline
\multicolumn{1}{|c|}{\textit{Neural Kinematics}}         & \multicolumn{1}{r|}{97.17}              & \multicolumn{1}{r|}{79.23}              & \multicolumn{1}{r|}{65.05}              & \multicolumn{1}{r|}{\textbf{40.0}}      & \multicolumn{1}{r|}{70.64}            \\ \hline
\end{tabular}

\caption{Percentage of successfully reaching the target point for different methods, where a success is being within 0.005 of the target. In bold is the best performing method for a given distance. Overall represents performance regardless of distance to target.  }
\label{tab:pttoptdist}
\end{table}

\begin{table}[]
\begin{tabular}{cccccc}
\multicolumn{1}{l}{}                                     & \multicolumn{5}{c}{\textbf{Initial Distance}} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Model}}}            & \multicolumn{1}{c|}{\textit{0.0 - 1.0}} & \multicolumn{1}{c|}{\textit{1.0 - 2.0}} & \multicolumn{1}{c|}{\textit{2.0 - 3.0}} & \multicolumn{1}{c|}{\textit{3.0 - 4.0}} & \multicolumn{1}{c|}{\textit{Overall}} \\ \hline
\multicolumn{1}{|c|}{\textit{Inverse Jacobian}}          & \multicolumn{1}{c|}{80.21}               & \multicolumn{1}{c|}{89.82}               & \multicolumn{1}{c|}{78.88}                & \multicolumn{1}{c|}{76.87}                & \multicolumn{1}{c|}{82.64}            \\ \hline
\multicolumn{1}{|c|}{\textit{Broyden}}                   & \multicolumn{1}{c|}{28.12}               & \multicolumn{1}{c|}{15.27}               & \multicolumn{1}{c|}{3.45}                 & \multicolumn{1}{c|}{0.00}                 & \multicolumn{1}{c|}{9.36}             \\ \hline
\multicolumn{1}{|c|}{\textit{Finite Difference}}         & \multicolumn{1}{c|}{23.96}               & \multicolumn{1}{c|}{9.67}                & \multicolumn{1}{c|}{1.29}                 & \multicolumn{1}{c|}{0.00}                 & \multicolumn{1}{c|}{6.09}             \\ \hline
\multicolumn{1}{|c|}{\textit{Local Linear}}              & \multicolumn{1}{c|}{45.83}               & \multicolumn{1}{c|}{41.73}               & \multicolumn{1}{c|}{32.33}                & \multicolumn{1}{c|}{14.29}                & \multicolumn{1}{c|}{34.45}            \\ \hline
\multicolumn{1}{|c|}{\textit{Multitask Neural Jacobian}} & \multicolumn{1}{c|}{50.00}               & \multicolumn{1}{c|}{24.17}               & \multicolumn{1}{c|}{10.56}                & \multicolumn{1}{c|}{0.00}                 & \multicolumn{1}{c|}{17.45}            \\ \hline
\multicolumn{1}{|c|}{\textit{Neural Jacobian}}           & \multicolumn{1}{c|}{39.58}               & \multicolumn{1}{c|}{22.90}               & \multicolumn{1}{c|}{9.05}                 & \multicolumn{1}{c|}{3.40}                 & \multicolumn{1}{c|}{15.91}            \\ \hline
\multicolumn{1}{|c|}{\textit{Neural Kinematics}}         & \multicolumn{1}{c|}{\textbf{70.83}}      & \multicolumn{1}{c|}{\textbf{45.80}}      & \multicolumn{1}{c|}{\textbf{36.21}}       & \multicolumn{1}{c|}{\textbf{17.01}}       & \multicolumn{1}{c|}{\textbf{40.09}}   \\ \hline
\end{tabular}
\caption{Percentage of successfully reaching the target point for different methods on multi-point simulation. The success is being within 0.05 of the target. In bold is the best performing method for a given distance. Overall represents performance regardless of distane to target. \rrr combined 2 tables in 1 to save space ... \kkk }
\label{tab:multi-pt-dist}
\end{table}



==> supplementary_files/InvJacDets.tex <==
\section{Inverse Jacobian Derivation for Reacher}

Here we include the equations that describe the inverse Jacobian controller used for the Kinova environment. With two planar rotation joints the position of the end-effector can be described by the following equations:
\begin{equation}
    x_{e} = 
    \begin{bmatrix}
        x\\[\jot]
        y\\[\jot]
    \end{bmatrix}
        =
        \begin{bmatrix}
         L_{1} cos(q_{1}) + L_{2} cos(q_{1} + q_{2})\\L_{1}sin(q_{1}) + L_{2} sin(q_{1} + q_{2})
        \end{bmatrix}
\end{equation}.

Using the equation in the main paper by taking the derivative with respect to time we end up with the following controller: 
\begin{equation}
 \frac{\partial x_{e}}{\partial t} =
        \begin{pmatrix}
         -L_{1}sin(q_{1}) - L_{2} sin(q_{1} + q_{2}) &
         - L_{2} sin(q_{1} + q_{2})
         
         \\
         L_{1} cos(q_{1}) + L_{2} cos(q_{1} + q_{2}) &
         L_{2} cos(q_{1} + q_{2})
        \end{pmatrix}
        \begin{pmatrix}
            \dot{q_{1}} \\  \dot{q_{2}}
        \end{pmatrix}.
\end{equation}
We exclude writing $J^{-1}$, but note that it can be found analytically using the fact $J$ is a 2-by-2 matrix.

\begin{equation}
    \min_{q} ||x^{*} - f(q)||^{2}_{2}
\end{equation}

==> supplementary_files/additional_exp_folder/jacobian_conditioning_of_environment.tex <==
\subsection{Jacobian Conditioning of Environments}

\begin{table}[]
\begin{tabular}{c|c|c|c|c|}
\cline{2-5}
                                                         & \multicolumn{2}{c|}{Single Point} & \multicolumn{2}{c|}{Multiple Points} \\ \cline{2-5} 
                                                         & mean       & standard deviation   & mean           & standard deviation  \\ \hline
\multicolumn{1}{|c|}{\textbf{Broyden}}                   & 11.658     & 25.373               & 6.070931e+14   & 5.305740e+15        \\ \hline
\multicolumn{1}{|c|}{\textbf{Finite Difference}}         & 15.933     & 0.000                & 3.785613e+16   & 1.600000e+01        \\ \hline
\multicolumn{1}{|c|}{\textbf{KNN Local Linear}}          & 141.677    & 40410.916            & 1.846220e+02   & 3.844440e+02        \\ \hline
\multicolumn{1}{|c|}{\textbf{Multitask Neural Jacobian}} & 3.290      & 1.795                & 1.085200e+01   & 3.987000e+00        \\ \hline
\multicolumn{1}{|c|}{\textbf{Neural Jacobian}}           & 5.101      & 4.067                & 1.520790e+02   & 1.313760e+02        \\ \hline
\multicolumn{1}{|c|}{\textbf{Neural Kinematics}}         & 5.428      & 4.463                & 2.007880e+02   & 1.743080e+02        \\ \hline
\multicolumn{1}{|c|}{\textbf{True Jacobian}}             & 5.025      & 4.456                & 1.877426e+08   & 1.278614e+08        \\ \hline
\end{tabular}
\caption{The average Jacobian condition number for each environment by algorithm. We found that between methods that there was not a significant difference, but between environment the conditioning was much more notable.}
\label{tab:jacobiancond}
\end{table}

In this experiment we looked at the matrix condition number for the Jacobians at each step of control for all algorithms and for each step of control. The condition number gives us an idea of how close to singularities, or linear dependence our matrices are \cite{heath1996scientificcomputing}. Closer to 1 suggest better conditioned matrices that are robust to noise. For this analysis we averaged across all Jacobian calculations in our experiments. These included each step of a trajectory across all collected trajectories. We note this does not give a complete picture of conditioning between algorithms, and is primarily to illustate the challenges between the single point and multi point experiments.  The results are included in Table~\ref{tab:jacobiancond}. Between algorithms we observed some noticeable differences between average Jacobian conditioning for different approximations in the single point case. Across environments, the much large magnitudes of condition numbers in the multi-point environment demonstrates the difficulty of this task, where all algorithms are much more poorly conditioned for the task, including the true Jacobian. 

==> supplementary_files/additional_exp_folder/knn_tuning_experiment.tex <==
\subsection{Sensitivity of Number of Neighbours}

In this section we provide results from tuning the number of neighbours in our KNN Neural Jacobian method. We only conducted the experiment on the multi-point environment using the same trajectories in our control experiments. The hyperparameters are almost entirely the same as our other multi-point experiments. One exception is that we use 50 epochs to train over as opposed to the 40 in the original experiment. We increased the number of epochs to allow sufficient time for the model to converge, even if the best performance on the validation set occurred much earlier. We tried values 2, 4, 8, 16, 32, 64 for the neighborhood. We did not try a higher number of neighbors as our current results suggest the number of neighbors is not that sensitive, and with our implementation we stored the dataset in memory so the cost was too much. 
We also tuned over the number of neighbors in the local linear baseline. We include the percentage of successful controls to the target point and the Condition number. We also plotted the Jacobian error, but our results were generally consistent with previous work with the Local linear method. An interesting exception was our results with eight neighbors. We found that our Jacobian estimates exploded. We conjecture that this is because when the number of neighbors is small 

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{diagrams/sensitivity_to_knn/knn-neuraljacobian-custom_multi_pt_error_curves.pdf}  
  \caption{Vanilla KNN Neural Jacobian}
  \label{fig:betatuningeuclideandistsinglepoint}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{diagrams/sensitivity_to_knn/multitask-knn-neuraljacobian-custom_multi_pt_error_curves.pdf}  
  \caption{Multitask KNN Neural Jacobian}
  \label{fig:betatuningeuclideandistMultipoint}
\end{subfigure}

\caption{Performance of different neighborhood sizes for the KNN Neural Jacobian method on the Multiple Point environment.}
\label{fig:knnsensitivityeuclideandist}
\end{figure}


\begin{table}[]
\centering
\setlength{\tabcolsep}{3 pt}
\renewcommand{\arraystretch}{0.9}
{\small
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
           & \multicolumn{5}{c|}{\textbf{KNN Neural Jacobian}}                                                         &           & \multicolumn{5}{c|}{\textbf{Multitask KNN Neural Jacobian}}                                               \\ \hline
\textbf{K} & \textbf{0.0 - 1.0 m} & \textbf{1.0 - 2.0 m} & \textbf{2.0 - 3.0 m} & \textbf{3.0 - 4.0} & \textbf{Overal} & \textbf{} & \textbf{0.0 - 1.0 m} & \textbf{1.0 - 2.0 m} & \textbf{2.0 - 3.0 m} & \textbf{3.0 - 4.0} & \textbf{Overal} \\ \hline
2          & 68.02                & 49.51                & 39.61                & 26.00              & 43.81           &           & 88.30                & 74.29                & 59.30                & 41.70              & 64.83           \\ \hline
4          & 70.94                & 49.26                & 38.87                & 25.25              & 43.56           &           & 89.93                & 70.75                & 56.10                & 38.32              & 61.91           \\ \hline
8          & 65.42                & 47.70                & 37.56                & 24.14              & 41.82           &           & 88.83                & 72.61                & 55.33                & 40.81              & 62.49           \\ \hline
16         & 57.03                & 50.19                & 34.64                & 15.75              & 39.63           &           & 89.55                & 72.09                & 57.20                & 46.54              & 63.92           \\ \hline
32         & 59.88                & 50.21                & 34.42                & 20.46              & 40.42           &           & 90.51                & 74.19                & 58.65                & 42.51              & 64.82           \\ \hline
64         & 71.27                & 48.54                & 32.60                & 18.19              & 39.75           &           & 90.32                & 77.42                & 60.52                & 41.28              & 66.59           \\ \hline
\end{tabular}
}
\label{tab:knnsensitivity}
\caption{Success percentages averaged from 0.0 - 0.25 with increments of 0.001 steps.}
\end{table}

==> supplementary_files/additional_exp_folder/multi_task_tuning.tex <==
\section{Multitask Jacobian Parameter Comparisons}

In this section we include additional results when we investigated tuning the weighting term $\beta$ for the Multitask Neural Jacobian. Our experimental set-up was the same as described previously for the simulators. We only consider comparing the Multitask Neural Jacobian against each other. When $\beta=0.0$ this is the same as the original Neural Jacobian. 

Decreases in the Euclidean distance (meters) to the target are visualized in Figure~\ref{fig:betatuningeuclideandist}. This plot suggests that increasing $\beta$ seems to help in the multi-point environment for the closer targets but overall differences are relatively minute. We also include the percentages of successes, which was calculated the same way for our other experiments, in Table~\ref{tab:tuningbetasuccesses}. These results show similar results reported in our main paper, where the main benefits of the Multitask Neural Jacobian seem more evident in the multi-point environment. For the single point case,  even for smaller $\beta$ negatively, impact performance.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{diagrams/beta-tuning/singlepoint/beta_tuning_pt_to_pt_error_curves.pdf}  
  \caption{Single Point Alignment}
  \label{fig:betatuningeuclideandistsinglepoint}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{diagrams/beta-tuning/multipoint/beta_tuning_multi_pt_error_curves.pdf}  
  \caption{Multi-point alignment}
  \label{fig:betatuningeuclideandistMultipoint}
\end{subfigure}

\caption{Euclidean distance (meters) to target with varying the weighting term in the Multitask Neural Jacobian. Plotted are the average performances across trajectories separate by initial starting distances. The filled area is the standard error of the mean. For the multi-point case distance is the sum of each point's distance to their respective targets.}
\label{fig:betatuningeuclideandist}
\end{figure}


\begin{table}[]
\centering
\setlength{\tabcolsep}{3 pt}
\renewcommand{\arraystretch}{0.9}
{\small
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-12}
\multicolumn{1}{l|}{\textbf{}}         & \multicolumn{11}{c|}{\textbf{Initial Euclidean Distance (meters)}}                                                                                                                                                      \\ \cline{2-12} 
\multicolumn{1}{l|}{}                  & \multicolumn{5}{c|}{\textbf{Single Point}}                                                           &           & \multicolumn{5}{c|}{\textbf{Multiple Points}}                                                        \\ \hline
\multicolumn{1}{|c|}{\textbf{$\beta$}} & \textbf{0.0 - 0.5} & \textbf{0.5 - 1.0} & \textbf{1.0 - 1.5} & \textbf{1.5 - 2.0} & \textbf{Overall} &           & \textbf{0.0 - 1.0} & \textbf{1.0 - 2.0} & \textbf{2.0 - 3.0} & \textbf{3.0 - 4.0} & \textbf{Overall} \\ \hline
\multicolumn{1}{|c|}{\textbf{0.0}}     & \textbf{98.96}     & 85.53              & \textbf{74.75}     & 41.84              & \textbf{77.40}   & \textbf{} & 58.56              & 40.19              & 22.63              & 9.09               & 30.23            \\ \hline
\multicolumn{1}{|c|}{\textbf{0.05}}    & 98.94              & 83.26              & 74.64              & 37.60              & 76.02            & \textbf{} & 58.56              & 40.19              & 22.63              & 9.09               & 30.23            \\ \hline
\multicolumn{1}{|c|}{\textbf{0.1}}     & 98.92              & \textbf{86.03}     & 69.66              & \textbf{45.18}     & 75.86            & \textbf{} & 61.21              & 40.58              & 24.20              & 10.19              & 31.41            \\ \hline
\multicolumn{1}{|c|}{\textbf{0.2}}     & 98.97              & 84.97              & 69.86              & 42.94              & 75.30            & \textbf{} & 57.47              & 35.84              & 22.81              & \textbf{10.74}     & 28.88            \\ \hline
\multicolumn{1}{|c|}{\textbf{0.4}}     & 98.00              & 85.58              & 73.23              & 42.48              & 76.77            & \textbf{} & 66.53              & 43.54              & 25.70              & 10.73              & \textbf{33.64}   \\ \hline
\multicolumn{1}{|c|}{\textbf{0.8}}     & 98.82              & 84.78              & 71.07              & 43.08              & 75.72            & \textbf{} & 63.96              & 42.56              & \textbf{26.42}     & 7.40               & 32.92            \\ \hline
\multicolumn{1}{|c|}{\textbf{1.0}}     & 98.82              & 83.38              & 70.53              & 39.07              & 74.52            & \textbf{} & 63.10              & \textbf{44.91}     & 25.78              & 5.58               & 33.17            \\ \hline
\multicolumn{1}{|c|}{\textbf{1.6}}     & 98.44              & 84.70              & 65.85              & 35.82              & 72.67            & \textbf{} & \textbf{69.80}     & 39.61              & 25.29              & 9.04               & 32.12            \\ \hline
\end{tabular}
}
\caption{Percentage of successfully reaching targets for different values of $\beta$ in Multitask Neural Jacobian method. We use the average success percentages for thresholds from 0.0m - 0.1m from target for single-point  and the AUC for 0.0m - 0.25m for multi-point. In bold are the best performance for each distance. In multi-point setting the distance is the sum of distances for all points to their respective targets.}
\label{tab:tuningbetasuccesses}
\end{table}

==> supplementary_files/additional_experiments.tex <==
\input{supplementary_files/additional_exp_folder/multi_task_tuning}
\input{supplementary_files/additional_exp_folder/jacobian_conditioning_of_environment}
\input{supplementary_files/additional_exp_folder/knn_tuning_experiment}

==> supplementary_files/baseline_methods.tex <==
\section{Baseline Methods}
In this section, we describe the details of each of the baseline methods we compared against. This included the true Jacobian, finite difference method~\cite{jagersand96visualservoing}, the Broyden method~ \cite{jagersand96visualservoing}, and the Local Linear method \cite{farahmand2007globaluvs}. As the Broyden method and finite difference method are closely related, they are described together.

\subsection{True Robotic Jacobian}

Here we include relevant equations that describe the true Jacobian for the 2-DOF environment we mapped to the Kinova. With two planar rotation joints the position of the end-effector can be described by the following equations:
\begin{equation}
    x = 
        \begin{bmatrix}
         L_{1} cos(q_{1}) + L_{2} cos(q_{1} + q_{2})\\L_{1}sin(q_{1}) + L_{2} sin(q_{1} + q_{2})
        \end{bmatrix}
\end{equation}.

Using the equation for robotic motion in the main paper, when we  differentiate with respect to time, we get the following Jacobian: 
\begin{equation}
 \dot{x} =
        \begin{pmatrix}
         -L_{1}sin(q_{1}) - L_{2} sin(q_{1} + q_{2}) &
         - L_{2} sin(q_{1} + q_{2})
         \\
         L_{1} cos(q_{1}) + L_{2} cos(q_{1} + q_{2}) &
         L_{2} cos(q_{1} + q_{2})
        \end{pmatrix}
        \begin{pmatrix}
            \dot{q_{1}} \\  \dot{q_{2}}
        \end{pmatrix} 
\end{equation}
Here, $L_{1}$ and $L_{2}$ our the lengths of the robot links. We exclude writing $J^k{-1}$, but note that it can be found analytically using the fact $J$ is a 2-by-2 matrix. For our simulators, we found that analytically writing the Jacobian would be fairly complex for the 7 DOF manipulator, and instead we used a backpropagation library to handle calculating the Jacobian \cite{jax2018github}.



\subsection{k Nearest Neighbor Local Linear Jacobian Estimation}
Previous research on Jacobian approximation has utilized the observation that the Jacobian is a hyperplane at the instantaneous point of evaluation \cite{farahmand2007globaluvs}. This work considered directly fitting such a hyper-plane utilizing the assumption that the equations of robot motion can be approximated as finite differences $\Delta x \approx J(q_{t}) \Delta q$ for time step $t$ in a trajectory, leading to the following objective: 
\begin{equation}
    \min_{J} \sum^{k}_{i=1}\sum^{k}_{j=1}|| \Delta x_{ij} - J\Delta q_{ij} ||_{2}^{2},
\end{equation}
where $\Delta x_{ij}$ and $\Delta q_{ij}$ are the finite difference between the k-nearest neighbor (k-NN) points to the current angles $q_{t}$ we want to calculate the Jacobian. This objective function is then optimized online when controlling the robot, and can be anlytically solved by differentiating with respect to the Jacobian J. This method requires storing all the interactions with the robot to select the k-NN neighbors to be optimized over. In our experiments we used $k=50$ for evaluation based on previous works experimental results \cite{farahmand2007globaluvs}.

\subsection{Broyden Jacobian Estimation}

One classic approach to estimating the Jacobian is by making small, independent movements of each joint from some initial pose \cite{ramirez2018libraryUVS}. In a 2-DOF planar reaching environment, this matrix is found as follows:   
\begin{equation}
    J \approx \hat{J}=
    \begin{pmatrix}
        \frac{x^{t} - x^{0}}{q^{t}_{1} - q^{0}_{1}} & \frac{x'^{t} - x^{0}}{ q^{t}_{2} - q^{0}_{2}}\\[\jot]
        \frac{y^{t} - y^{0}}{q^{t}_{1} - q^{0}_{1}} & \frac{y'^{t} - y^{0}}{ q^{t}_{2} - q^{0}_{2}}\\[\jot]
    \end{pmatrix}.
\end{equation}
Here, $t$ is the position after some amount of movement. Note that, for each columns approximation we assume the same initial position $(x^{0}, y^{0})$. We only include the coordinates for a 2-dimensional point, but the matrix is similar for 3D points as well. For each column of this matrix, we move the joints sufficiently far such that the change in position is non-negligible. To improve the estimate of this Jacobian we can then make Broyden updates of the Jacobian as follows:
\begin{equation}
 \hat{J}_{k+1} = \hat{J}_{k} + \alpha \frac{(\Delta e - \hat{J}_{k}\Delta q) \Delta q^{T}}{||\Delta q||_{2}^{2}}.
\end{equation}
Here $\Delta$ is for changes from the last tracked measurements, and $e = x^{*} - x$. A limitation of the Broyden update is it requires the change in joint angles $\Delta q$ be sufficiently large. In our experiments for the Broyden method, we only take the update if $||\Delta q||_{2}^{2} \geq 0.01$ and used $\alpha=0.1$ when updating the approximation $\hat{J}_{k}$.  

==> supplementary_files/environment_details.tex <==
\section{Environment Details}

\begin{table}[]
\centering
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
\textbf{}                                            & \textit{\textbf{$x$}} & \textit{\textbf{$\cos(q)$}} & \textit{\textbf{$\sin(q)$}} & \textit{\textbf{$\dot{q}$}} & \textit{\textbf{$x^{*}$}} & \textit{\textbf{$s$}} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Single Point}}} & 3                     & 7                           & 7                           & 7                           & 3                         & 27                    \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Multi Point}}}  & 12                    & 7                           & 7                           & 7                           & 12                        & 45                    \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Kinova}}}       & 2                     & 2                           & 2                           & 2                           & 2                         & 10                    \\ \hline
\end{tabular}
\caption{Dimensions of different aspects of the robot state $s$ for each environment. This includes end-effector location $x$, joint angles $q$, joint velocities $\dot{q}$, and target location $x^{*}$, where $s$ is the sum of these dimensions. Commands sent to the environments were joint velocities $\dot{q}$.}
\label{tab:statedimensions}
\end{table}
We describe the details for our simulated and robotic environments in this section. All our environments are designed similarly to a reinforcement learning gym \cite{brockman2016OpenAIGYM} where the actions are joint velocities $\dot{q}$ and we receive the robot state as a vector $s$. Each environment consists of the same robotic information, only differing in the dimensions of each feature. We list these dimensions for each environment in Table~\ref{tab:statedimensions}.

In both simulated and robotic environments, we utilize the Kinova's kinematics equations for generating the location of targets. As mentioned in the background section, we used the Denavit-Hartenberg (DH) parameters for the Kinova's kinematics. The DH matrix is as follows:
\begin{equation}
 ^{i-1}T_{i} =
\begin{pmatrix}
 \cos(q_{i}) & -\cos(\alpha_{i})\sin(q_{i}) & \sin(\alpha_{i})\sin(q_{i}) & a_{i}\cos(q_{i})\\
 \sin(q_{i}) & \cos(\alpha_{i})\cos(q_{i}) & -\sin(\alpha_{i})\cos(q_{i}) & a_{i}\sin(q_{i})\\
 0 & \sin(\alpha_{i}) & \cos(\alpha_{i}) & d_{i}\\
 0 & 0 & 0 & 1 
\end{pmatrix}.
\end{equation}
For each transformation $^{i-1}T_{i}$ of the Kinova, the values can be found in Table~\ref{tab:kinovadhvalues}. 

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.7\linewidth]{./diagrams/onepointsimulator.pdf}  
  \caption{Point to Point Environment}
  \label{fig:1ptsimulator}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.7\linewidth]{diagrams/fourpointsimulator.pdf}  
  \caption{Position and Orientation Environment}
  \label{fig:4ptsimulator}
\end{subfigure}
\caption{Visualization of kinematic simulators. The objective in both simulators is to align robot points (orange) to match exactly with corresponding target points (blue) }
\label{fig:simulators}
\end{figure}

\paragraph{Simulator Details} Our simulator environments are visualized in Figure~\ref{fig:simulators}, and were implemented with the DH parameter values in Table~\ref{tab:kinovadhvalues}. They only differ in the number of points we wish to move to a target position. In the single point case, we only translate a single homogeneous vector $p=[0,0,0,1]$ with the kinematics equations to represent the end-effector. In the multi-point case we include 3 additional vectors, where each is a scaled unit-vectors of the orientation for the x, y, and z axis. We found using one-tenth of a unit vector the best for visualizing the points representing orientation (e.g. $p_{z}=[0, 0, .1, 1]$ as opposed to $p_{z}=[0, 0, 1, 1]$). When joint velocities are sent, the current joint values are updated as $q_{t+1} = q_{t} + \Delta t \dot{q_{t}}$, where $\Delta t=0.05 \text{(seconds)}$ represents our simulated time. The position of the robot is then updated and a new state vector is sent with the updated information to our controller.

\begin{table}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{i}    & \textbf{$\alpha_{i}$ (radians)} & \textbf{$a_{i}$(m)} & \textbf{$d_{i}$(m)} & \textbf{$q_{i}$ (radians)} \\ \hline
0 (from base) & $\pi$                           & 0.0                 & 0.0                 & 0                               \\ \hline
1             & $\pi / 2$                       & 0.0                 & -(0.1564 + 0.1284)  & $q_{1}$                         \\ \hline
2             & $\pi / 2$                       & 0.0                 & -(0.0054 + 0.0064)  & $q_{2} + \pi$                   \\ \hline
3             & $\pi / 2$                       & 0.0                 & -(0.2104 + 0.2104)  & $q_{3} + \pi$                   \\ \hline
4             & $\pi / 2$                       & 0.0                 & -(0.0064 + 0.0064)  & $q_{4} + \pi$                   \\ \hline
5             & $\pi / 2$                       & 0.0                 & -(0.2084 + 0.1059)  & $q_{5} + \pi$                   \\ \hline
6             & $\pi / 2$                       & 0.0                 & 0.0                 & $q_{6} + \pi$                   \\ \hline
7             & $\pi$                           & 0.0                 & -(0.1059 + 0.0615)  & $q_{7} + \pi$                   \\ \hline
\end{tabular}
\caption{Table of DH parameter values for the Kinova robot \cite{kinova}. We utilize these numbers for calculating the target location, position of our simulators, and for calculating the true Jacobian.}
\label{tab:kinovadhvalues}
\end{table}

\paragraph{Kinova Details}
\begin{figure}
    \centering
    \includegraphics[width=.3\linewidth]{diagrams/vs_image.png}
    \caption{Image of the Kinova Gen 3 light robot used for experiments. Visualization of the tool tip (blue orange circle) and target position (green) in image are to illustrate fundamental idea of the control task. In experiments we work in robot coordinate system.}
    \label{fig:Kinova}
\end{figure}


For our Kinova experiments, we derived the DH parameters for a 2 degree-of-freedom (DOF) planar manipulator. The kinematic transformations can be found in \citet[Chapter 3]{craig1989IntroRobotics} for this planar case. This required transforming the Kinova's coordinate system to align with our planar forward kinematics equations. Specifically, we converted from the Kinova's z-x plane to a x-y coordinate frame, by subtracting an offset of 0.7052 from the Z axis and treated it as our X coordinates while treating the Kinova x coordinate as our y axis. We then interpreted the Kinova's 4th link of length 0.3143 meters as the first link in our 2-DOF robot,  and the Kinova's 6th joint of length 0.1774 meters as the second link. We interacted with the Kinova using the publicly available the Kinova Robotic Operating System (ROS) bindings \cite{ros2018ROS,kinovakortex}. The all features of the robot's state was sensory information from the Kinova. Similarly, joint velocity commands were sent through the ROS bindings. We operated our the Kinova at approximately 20 Hz which corresponded to about 10 seconds for real-time evaluation on the robot per trajectory. 

==> supplementary_files/experiment_details.tex <==
\section{Experiment Details}

\begin{table}[]
\centering
{\small
\begin{tabular}{c|c|c|c|}
\cline{2-4}
\textbf{}         & \textbf{Single  Point (Simulation)} & \textbf{Multi-Point (Simulation)} & \multicolumn{1}{l|}{\textbf{Single Point (Kinova)}} \\ \hline
\multicolumn{1}{|l|}{\# of Training Epochs} & 30                                  & 40                                & 45                                                  \\ \hline
\multicolumn{1}{|c|}{\# Hidden Layers}      & 2                                   & 4                                 & 1                                                   \\ \hline
\multicolumn{1}{|c|}{Hidden Layer Size}     & \multicolumn{3}{c|}{100}                                                                                                      \\ \hline
\multicolumn{1}{|c|}{Activation Function}   & \multicolumn{3}{c|}{Relu}                                                                                                     \\ \hline
\end{tabular}
}
\caption{Neural network hyperparameters for each experiment. }
\label{tab:networkparams}
\end{table}

\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Single Point Distances} & \textbf{Counts} & \textbf{Multi-point Distances} & \textbf{Counts} \\ \hline
0.0 - 0.5                       & 106             & 0.0 - 1.0                      & 96              \\ \hline
0.5 - 1.0                       & 414             & 1.0 - 2.0                      & 393             \\ \hline
1.0 - 1.5                       & 455             & 2.0 - 3.0                      & 464             \\ \hline
1.5 - 2.0                       & 125             & 3.0 - 4.0                      & 147             \\ \hline
\end{tabular}
\caption{Trajectory counts for simulation experiments by initial distances to target}
\end{table}

In this section, we provide additional details on our experimental step-up. We list our neural network hyperparameters in Table~\ref{tab:networkparams}. We used the Adam optimizer for all experiments with $\beta_{1}=0.9$, $\beta_{2}=0.999$, and learning rate $\alpha=0.001$. These were the default parameters in the deep learning framework we implemented our methods with \cite{paszke2019pytorch}. In all our experiments we used a mini-batch size of 32 for training all neural methods.

We collected trajectories as training data for each experiment. We ran an Ornstein and Uhlenbeck process \cite{uhlenbeck1930brownianmotion} with the following parameters: $\sigma=1.00$, $\mu=0.00$, $\theta=0.15$, $\theta$ here is not the same as model parameters. In our single point simulation, we used a training dataset of 100,000 (1000 trajectories of 100 time-steps each), and for the multi-point environment we used a training dataset of 200,000 (2000 trajectories of 100 times-steps). We re-used each random seeds training dataset for all models in our experiments. The one exception is the Neural Jacobian models which collected additional trajectories before training because each datum required sub-sequent steps to formulate a training example. 

For evaluation in both simulators, we generated 110 random targets for each of the 10 random seeds for a total of 1100 targets used for reported results. The targets were generated by uniform sampling in the joint angles and transforming them with the Kinova kinematics. This does not correspond with uniform sampling of the Cartesian work-space because of the transformations from the kinematic equations. We allowed each model 200 time-steps to reach the target which corresponded to 10 seconds of simulated time. In our experiments we set the gain value $\lambda=1.0$ which we found worked well for all methods.
 
 On the Kinova, we collected 10,000 training examples (100 trajectories of 100 time-steps) with the same Ornstein and Uhlenbeck process parameters. Unlike the simulator experiments, we re-used the same 10,000 samples for each random seed, meaning the random seed mostly affected initialization for the neural network parameters. We generated 25 random targets for each seed from the Kinova's kinematics bounded between $[-2.0, 2.0]$ for the first control joint and $[-1.5, 1.5]$ of the second joint. We only worked with 2 Joints of the Kinova, and discuss details of this in the next section. Targets were reused between all models considered. During evaluation, we used a gain $\lambda=0.9$ for for evaluation, but collected data with $\lambda = 1.0$.

==> supplementary_files/jacobian_histogram.tex <==
\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{diagrams/pt_to_pt_sim_diagrams/pt_to_pt_jacobian_hist.pdf}  
  \caption{Single Point Alignment}
  \label{fig:frobenius_single_histogram}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{diagrams/multi_point_diagrams/multi_pt_jacobian_hist.pdf}  
  \caption{Multi-point alignment}
  \label{fig:frobenius_multi_histogram}
\end{subfigure}
\caption{Frobenius distance of approximated Jacobians compared to the true Kinematics Jacobian over trajectories. Plots are of mean performance with standard-error of the mean.}
\label{fig:frobenius_histograms}
\end{figure}

Technically, the Frobenius distance between the true Jacobian and approximated Jacobians are not dependent on time of the trajectory being only functions of the joint angles. To see better see the distribution of Frobenius distance between Jacobian approximations, we plot histograms to see the variance of our approximations. These are available in Figure~\ref{fig:frobenius_histograms}. The Neural Kinematics model seems to be quite peaked in it's predictions for varying joint angles. The Neural Jacobian seems accurate as we move to the more complex environments, but in the single point environment is closer in approximation compared to the local linear models. 

==> supplementary_files/violin_plots_to_target.tex <==
\section*{Final Error Distribution}

These are just additional plots for our simulation results. Figure~\ref{fig:violint_pt_to_pt} shows the spread of the final euclidean distance to the target. 
\begin{figure}[ht]
    \centering
\includegraphics[width=\linewidth]{diagrams/pt_to_pt_sim_diagrams/pt_to_pt_violion_end_position.pdf}  
  \caption{Violin Plots of Final Positions. Plots Closer to zeros imply trajectories more likely to each target with method.}
    \label{fig:violint_pt_to_pt}
\end{figure}
